Flowco: Rethinking Data Analysis in the Age of LLMs

Conducting data analysis typically involves authoring code to transform, visualize, analyze, and interpret data. Large language models (LLMs) are now capable of generating such code for simple, routine analyses. LLMs promise to democratize data science by enabling those with limited programming expertise to conduct data analyses, including in scientific research, business, and policymaking. However, analysts in many real-world settings must often exercise fine-grained control over specific analysis steps, verify intermediate results explicitly, and iteratively refine their analytical approaches. Such tasks present barriers to building robust and reproducible analyses using LLMs alone or even in conjunction with existing authoring tools (e.g., computational notebooks). This paper introduces Flowco, a new mixed-initiative system to address these challenges. Flowco leverages a visual dataflow programming model and integrates LLMs into every phase of the authoring process. A user study suggests that Flowco supports analysts, particularly those with less programming experience, in quickly authoring, debugging, and refining data analyses.

==> code_snippet.tex <==
\begin{MintedVerbatim}[commandchars=\\\{\}]
\PYG{c+c1}{\PYGZsh{} put all imports here}
\PYG{k}{def}\PYG{+w}{ }\PYG{n+nf}{select\PYGZus{}fortis}\PYG{p}{(}\PYG{n}{beaks}\PYG{p}{:} \PYG{n}{pd}\PYG{o}{.}\PYG{n}{DataFrame}\PYG{p}{)} \PYG{o}{\PYGZhy{}}\PYG{o}{\PYGZgt{}} \PYG{n}{pd}\PYG{o}{.}\PYG{n}{DataFrame}\PYG{p}{:}
\PYG{+w}{  }\PYG{l+s+sd}{\PYGZdq{}\PYGZdq{}\PYGZdq{}}
\PYG{l+s+sd}{  select fortis}

\PYG{l+s+sd}{  This function has the following behavior:}
\PYG{l+s+sd}{  \PYGZhy{} The the result output is a Pandas DataFrame containing a subset}
\PYG{l+s+sd}{    of rows from the `beaks` DataFrame where the species is \PYGZsq{}fortis\PYGZsq{}.}
\PYG{l+s+sd}{  \PYGZhy{} The the result DataFrame retains the same columns and column}
\PYG{l+s+sd}{    names as the `beaks` DataFrame.}

\PYG{l+s+sd}{  Args:}
\PYG{l+s+sd}{    beaks (DataFrame[}
\PYG{l+s+sd}{     \PYGZsq{}species\PYGZsq{}: str  \PYGZsh{} The species name as a string.}
\PYG{l+s+sd}{     \PYGZsq{}Beak length, mm\PYGZsq{}: float  \PYGZsh{} The length of the beak in millimeters.}
\PYG{l+s+sd}{     \PYGZsq{}Beak depth, mm\PYGZsq{}: float  \PYGZsh{} The depth of the beak in millimeters.}
\PYG{l+s+sd}{    ]): The structure of the dataset representing bird species and}
\PYG{l+s+sd}{        their beak dimensions.}

\PYG{l+s+sd}{      Preconditions:}
\PYG{l+s+sd}{      \PYGZhy{} beaks is the dataframe for the `beaks` dataset.}

\PYG{l+s+sd}{  Returns:}
\PYG{l+s+sd}{    DataFrame[}
\PYG{l+s+sd}{     \PYGZsq{}species\PYGZsq{}: str  \PYGZsh{} The species of the bird.}
\PYG{l+s+sd}{     \PYGZsq{}Beak length, mm\PYGZsq{}: float  \PYGZsh{} The length of the beak in millimeters.}
\PYG{l+s+sd}{     \PYGZsq{}Beak depth, mm\PYGZsq{}: float  \PYGZsh{} The depth of the beak in millimeters.}
\PYG{l+s+sd}{    ]: The output is a filtered DataFrame containing only rows where}
\PYG{l+s+sd}{       the species is \PYGZsq{}fortis\PYGZsq{}, retaining all original columns and}
\PYG{l+s+sd}{       column names.}
\PYG{l+s+sd}{  \PYGZdq{}\PYGZdq{}\PYGZdq{}}
  \PYG{c+c1}{\PYGZsh{} put code here}
  \PYG{o}{.}\PYG{o}{.}\PYG{o}{.}
\end{MintedVerbatim}


==> macros-orig.tex <==
\newcommand{\hl}[2]{{\color{#1}\bfseries #2}}
\usepackage{tabularx} % For formal tables
\usepackage{booktabs} % For formal tables
\usepackage[ruled]{algorithm2e} % For algorithms
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{titlesec}
\usepackage{minted}
\usepackage{tikz}

\usepackage{balance}       % to better equalize the last page
\usepackage[T1]{fontenc}   % for umlauts and other diaeresis
\usepackage{hyperref}

\usepackage{color}
\usepackage{booktabs}

\usepackage{microtype}        % Improved Tracking and Kerning
\usepackage{ccicons}          % Cite your images correctly!

\usepackage{cuted}
\usepackage{capt-of}

\usepackage{upquote}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{float}

\usepackage[most]{tcolorbox}

\newcommand\upquote[1]{\textquotesingle#1\textquotesingle}



\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{white},
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}

\definecolor{light-gray}{gray}{0.95}

\lstset{style=mystyle}
\definecolor{lightgray}{rgb}{0.83, 0.83, 0.83}

\usepackage{multirow}

\usepackage{blindtext}
\usepackage{subcaption}
\usepackage{caption}

\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{multicol}

\usepackage{appendix}

\usepackage{tikz}
\usetikzlibrary{positioning,arrows.meta,graphs,backgrounds,fit,calc,quotes,shapes.multipart}
\usepackage{pgfplots}
\usepackage{pgfplotstable}

\pgfplotsset{width=3.5cm,
    tick label style={font=\footnotesize}
}

\definecolor{tisanecodetop}{RGB}{74,63,106}
\definecolor{closecolor}{RGB}{225,93,87}
\definecolor{minimizecolor}{RGB}{245,215,90}
\definecolor{maximizecolor}{RGB}{111,208,74}


\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}

\newcommand{\diff}[1]{\textcolor{blue}{#1}}

\newcommand{\eunice}[1]{\hl{purple}{EJ: #1}}
\newcommand{\emery}[1]{\hl{blue}{EB: #1}}
\newcommand{\steve}[1]{\hl{violet}{SF: #1}}
\newcommand{\kayla}[1]{\hl{magenta}{KL: #1}}

\newcommand{\old}[1]{\hl{gray}{OLD: #1}}

\def\redacted{REDACTED FOR REVIEW}
\newcommand{\keyidea}{\textcolor{blue}}
\newcommand{\fillin}{\textcolor{red}}
\newcommand{\rr}{\textcolor{black}} % for Revise & Resubmit

\newcommand{\pythoness}{\textsc{Pythoness}}
\newcommand{\flowco}[0]{\textsc{Flowco}\xspace}
\renewcommand{\t}[1]{\texttt{#1}}
\newcommand{\dataflow}{dataflow\xspace}
\newcommand{\dataflowCaps}{Dataflow\xspace}

\newcommand{\shortquote}[1]{``\emph{#1}''}
\newcommand{\longquote}[1]{\vspace{-1pt}\begin{quote}``\emph{#1}''\end{quote}}
\newcommand{\longquoteEmphAdded}[1]{\vspace{-1pt}\begin{quote}``\emph{#1}'' (emphasis added).\end{quote}}
\newcommand{\theme}[1]{\vspace{-1pt}\subsubsection{#1} }
\newcommand{\groupingtheme}[1]{\subsubsection{\textbf{#1}} }

\def\lme{\texttt{lme4}\xspace}
\def\statsmodels{\texttt{statsmodels}\xspace}
\def\pymer{\texttt{pymer4}\xspace}

\def\sketch{Flowco\xspace}
\def\sketchs{Flowco's\xspace}
\def\dataSet{dataset\xspace}


\def\evalConceptualModels{\textbf{RQ1 - Conceptual model specification}\xspace}
\def\evalStatisticalModels{\textbf{RQ2 - Statistical model quality}\xspace}
\def\evalLearning{\textbf{RQ3 - Learning}\xspace}

\def\sectionautorefname{Section}
\renewcommand{\subsubsectionautorefname}{Subsubsection}

\def\etal{et al.\xspace}


\def\spaceHack{\relax}

\def\loosenessHack{\relax}

\newcommand{\mypara}[1]{\par\noindent\textbf{#1}\quad}

\newenvironment{compitem}
{ \begin{itemize}
    \setlength{\itemsep}{2pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}}
{ \end{itemize}}

\newenvironment{compenum}
{ \begin{enumerate}
    \setlength{\itemsep}{2pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}}
{ \end{enumerate}}


\usepackage{setspace}

\newcommand{\z}{\phantom{0}}

\newcommand{\p}{$\scriptsize{\pm}$}

\newcommand\colH[1]{\multicolumn{1}{c}{\textbf{#1}}}
\newcommand\colHR[1]{\multicolumn{1}{r}{\textbf{#1}}}
\newcommand\colsH[2]{\multicolumn{#1}{c}{\textbf{#2}}}

\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\newcommand{\assume}[1]{\tikz[baseline]\node[circle,inner xsep=2pt,inner ysep=0pt,
        draw=black,fill=white,scale=0.8,anchor=base] {#1};}
\newcommand{\valid}[1]{\tikz[baseline]\node[circle,inner xsep=2pt,inner ysep=0pt,
        draw=black,fill=gray!50!white,scale=0.8,anchor=base] {#1};}
\newcommand{\invalid}[1]{\tikz[baseline]\node[circle,inner xsep=2pt,inner ysep=0pt,
        draw=black,fill=white!30!white,scale=0.8,anchor=base] {#1};}
\def\yes{$\checkmark$}
\def\no{---}

\makeatletter
\newcommand\verytiny{\@setfontsize\verytiny{5pt}{6pt}} % Adjust 5pt/6pt as needed
\makeatother

\def\<#1>{\codeid{#1}}
\newcommand{\codeid}[1]{\ifmmode{\mbox{\small\ttfamily{#1}}}\else{\small\ttfamily #1}\fi}
\newcommand{\codeidsmall}[1]{\ifmmode{\mbox{\smaller\ttfamily{#1}}}\else{\smaller\ttfamily #1}\fi}


\NewTColorBox{mybox}{ O{red} m d"" !O{} }{
    enhanced,
    colframe=#1!25!white,
    colback=#1!5!white,
    coltitle=black,
    fonttitle=\bfseries,
    title=#2,
    beforeafter skip=0.25em,
    top=0em,
    bottom=0em,
    left=0.25em,
    right=0.25em,
    boxrule=0.5pt
}

\newenvironment{NodeTitle}[0]{
    \footnotesize
    \begin{mybox}[blue]{}
    \noindent \textbf{Summary}:
}{
    \end{mybox}
}

\newenvironment{NodeRequirements}[1][Requirements]{
    \footnotesize
    \begin{mybox}[teal]{}
    \noindent \textbf{#1}
}{
    \end{mybox}
}

\newenvironment{NodeCode}[1][Code]{
    \footnotesize
    \begin{mybox}[green]{}
    \noindent \textbf{#1}
}{
    \end{mybox}
}

\newenvironment{NodeOutput}[1][Output]{
    \footnotesize
    \begin{mybox}[yellow]{}
    \noindent \textbf{#1}
}{
    \end{mybox}
}

\newenvironment{NodeCheck}[1][Checks]{
    \footnotesize
    \begin{mybox}[orange]{}
    \noindent \textbf{#1}
}{
    \end{mybox}
}

\newenvironment{NodeTest}[1][Unit Tests]{
    \footnotesize
    \begin{mybox}[purple]{}
    \noindent \textbf{#1}
}{
    \end{mybox}
}

\newcommand{\unittest}[2]{
    \item \begin{tabular}[t]{@{}l@{~}l}
      \textbf{Input:} & #1 \\
      \textbf{Output:} & #2
    \end{tabular}
}

\NewTColorBox{amabox}{ O{red} m d"" !O{} }{
    enhanced,
    colframe=gray!25!white,
    colback=gray!5!white,
    coltitle=black,
    fonttitle=\bfseries,
    title=#1,
    beforeafter skip=0.25em,
    top=0em,
    bottom=0em,
    left=0.25em,
    right=0.25em,
    boxrule=0.5pt
}

\newcommand{\analyst}[0]{Alex\xspace}
